Neutron Star Powered Nebulae: A New View on Pulsar Wind Nebulae with the Fermi Gamma-ray Space Telescope

Pulsars are rapidly-rotating neutron stars born out of the death of stars. A diffuse nebula is formed when particles stream from these neutron stars and interact with the ambient medium. These pulsar wind nebulae (PWNe) are visible across the electromagnetic spectrum, producing some of the most brilliant objects ever observed. The launch of the Fermi Gamma-ray Space Telescope in 2008 has offered us an unprecedented view of the cosmic gamma-ray sky. Using data from the LAT on board Fermi, we search for new gamma-ray-emitting PWN. With these new observations, we vastly expand the number of PWN observed at these energies. We interpret the observed gamma-ray emission from these PWN in terms of a model where accelerated electrons produce gamma-rays through inverse Compton upscattering when they interact with interstellar photon fields. We conclude by studying how the observed PWN evolve with the age and spin-down power of the host pulsar.

==> chapters/offpeak/offpeak_auxiliary_description.tex <==
% \clearpage
\subsection{Description of Auxiliary information for Off-peak Analysis}
\label{off_peak_auxiliary}

A more complete list of the off-peak spectral and spatial 
results from the analysis described in \secref{unpulsed}
is contained
in a supplemental FITS table.
\tabref{off_peak_aux} describes each of its columns.

For sources reported with a PL spectral model,
the differential spectrum is defined as
\begin{equation}\eqnlabel{powerlaw_definition}
  \dnde = \fitsformat{Prefactor} \left(\frac{E}{\fitsformat{Scale}}\right)^{-\fitsformat{Index}}
\end{equation}
\fitsformat{Prefactor}, \fitsformat{Index}, and \fitsformat{Scale} are specified in the table.
For sources reported with a PLEC1 spectral model (\fitsformat{\PLSuperExpCutoff}), the differential spectrum is defined as:
\begin{equation}\eqnlabel{cutoff_powerlaw_definition}
  \dnde = \fitsformat{Prefactor} \left(\frac{E}{\fitsformat{Scale}}\right)^{-\fitsformat{Index}} \exp\left(-\frac{E}{\fitsformat{Energy\_Cutoff}}\right)
\end{equation}
and \fitsformat{Prefactor}, \fitsformat{Index}, \fitsformat{Scale}, and \fitsformat{Energy\_Cutoff} are specified in the table.

For the Crab Nebula and Vela-X, we took the spectral shape and
initial normalization from \citet{LAT_collaboration_crab_2012} and
\cite{FermiVelaX2nd} respectively
and fit only a
multiplicative offset (see \secref{off_peak_analysis}). For these two
sources, the differential spectrum was defined as
\begin{equation}\eqnlabel{filefunction_definition}
  \dnde = \fitsformat{Normalization} \left.\frac{dN}{dE}\right|_\mathrm{file}
\end{equation}
and the \fitsformat{Normalization} is defined in the auxiliary table.

% \clearpage
\begin{deluxetable}{p{1in} p{1in} p{3.5in}}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{Description of the Columns in the Off-Peak Auxiliary Fits Table
\tablabel{off_peak_aux}
}
\tablewidth{6in}
\input{OffPeak/tables/off_peak_auxiliary_table_description.tex}
\end{deluxetable}
\clearpage

